Gamma-ray Analysis of Pulsar Environments and Their Theoretical Explanation

Pulsars and their pulsar wind nebulae (PWNe) are unique laboratories for extreme astrophysical processes. This dissertation combines Fermi-LAT observations with a time-dependent leptonic PWN model (TIDE) to explore their gamma-ray emission. The model was validated on benchmark PWNe and applied to a systematic LAT search, leading to the discovery of new MeV-GeV candidates and the first population-level characterization. Several sources were modeled in detail, and predictions for potential TeV-emitting PWNe were tested against current and future observatories. Ultra-high-energy gamma-ray sources were also examined, revealing limits of standard leptonic scenarios. Beyond PWNe, stringent upper limits were obtained for the binary pulsar 1A 0535+262, and steady emission was detected from the globular cluster M5. Together, these results advance our understanding of pulsar environments and establish a framework for future multi-wavelength and next-generation gamma-ray studies.

==> Molecular_Cloud.tex <==
\chapter{Searching for gamma-ray emission from Swift J1818.0-1607 and unrepresented difusse emission in its projected vicinity}
\label{Clouds}
\textbf{\color{SectionBlue}\normalfont\Large\bfseries Contents of This Chapter}



\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Neutron stars are formed from the collapse of massive stars during supernova explosions. 
%
%A special class of these stars, which possess ultrahigh magnetic fields of $10^{14}-10^{15}$ G, is known as magnetars. 
%
%Furthermore, magnetars exhibit relatively long spin periods ($0.3-12$ s) and spin-down rates ($\sim 10^{-13}-10^{-11}$ s$^{-1}$), emit bright soft X-ray radiation, and display episodic short X-ray outbursts and even gamma-ray flares \citep{Ibrahim2023,Palmer2005}. 
%
%Given their extraordinary magnetic fields, magnetars are regarded as natural particle accelerators and are among the most promising candidates for the generation of fast radio bursts (FRBs). 
%
%The latter assumption is supported by the discovery of a bright FRB, which is possibly from the magnetar SGR J1935+2154 \citep{CHIME2020}. 
%
%However, to date, only pulsed radio and X-ray emissions have been identified, and all attempts to search for their pulsed $\gamma$-ray radiation have been unsuccessful (see, for example, \citet{Li2017}).

%
On 12 March 2020, the detection of a short X-ray burst of $\sim$ 0.1 s by NASA's Neil Gehrels Swift Observatory led to the discovery of a new magnetar, Swift J1818.0-1607 \citep{Evans2020}. 
%
%Its pulsed radio emission was subsequently observed in radio observations, 
Its pulsed radio emission was subsequently observed, classifying it 
%which classifies it 
as the fifth radio-loud magnetar \citep{Karuppusamy2020}. 
%
These radio observations yielded a rotation frequency of $f=0.7334110(2)$ Hz, a spin-down rate of $\dot{P}=8.16(2)\times10^{-11}$ s s$^{-1}$, and a dispersion measure of $DM=706(4)$ cm$^{-3}$ pc. These imply 
%from which they derived 
a characteristic age of $\tau_c \sim$ 265 yr, a dipolar surface magnetic field at the equator of $B_{sf}\sim3.4\times10^{14}$ G, and a distance of $D\sim4.8$ or $8.1$ kpc (utilizing different models of Galactic free electron density), respectively \citep{Champion2020,Karuppusamy2020,Esposito2020,Ibrahim2023}. 
%
It is noteworthy that, despite displaying some of the characteristics typically associated with other radio-loud magnetars, such as a high degree of linear polarization, its steep spectrum differs from the flat indices observed in the other four radio-loud magnetars. 
%
Instead, it exhibits a spectral profile more similar to that of a rotation-powered pulsar \citep{Lower2022}. 

%
%Given its relatively young age, this magnetar is the youngest of its kind and is therefore more likely to produce detectable $\gamma$-ray radiation. 
%
%In light of the aforementioned considerations, our first aim is to investigate the potential presence of $\gamma$-ray radiation from Swift J1818.0-1607, utilizing the \fermi Large Area Telescope (\lat, \citet{Atwood2009}) observational data. 
%
According to \citet{Li2017}, magnetars are not gamma-ray sources. However, the sample is still not numerous, and the fact that this pulsar is very young and have some differentiating properties promotes checking this conclusion in this case.
%
Motivated by the magnetar search in gamma-rays, utilizing the \fermi Large Area Telescope (\lat,\citet{Atwood2009}) observational data, we shall also critically study the region in its surrounding, which is plentiful of sources and possible counterparts at higher energies, but for which a detailed analysis of the possible implications of underrepresented molecular material is still lacking. 

%
%Despite the fact that our research yielded two new \fermi sources in this region (along with one that is not particularly significant), our research does not indicate a direct correlation with the magnetar. This outcome differs significantly from our initial objectives. 
%However, we view this as one of the most intriguing aspects of scientific research.

%In Section \ref{sec:data}, we provide a detailed description of the data set and the spatial and spectral analyses that were conducted. 
%Furthermore, the correlation between the detected $\gamma$-ray emission and the molecular clouds in this region is explored and presented in Section \ref{sec:CO}. 
%A comprehensive discussion of the results of our \fermi analyses is provided in Section \ref{sec:Discussion}. 
%In the final section, we present our conclusions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Data Analysis and Results}
\label{sec:data} % used for referring to this section from elsewhere
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Since its launch in 2008, \lat has been engaged in continuous observation and data recording, accumulating approximately 15 years worth of observational data.
%
%We used Pass8 SOURCE class data from August 4, 2008, to March 19, 2024, together with the processing tools contained in the \texttt{Fermitools} package\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/software/}} (v.2.2.0) and \texttt{Fermipy} (v.1.2.0, \citet{Wood2017}),
%
%and the latest version of the \lat source catalog (4FGL-DR4, \citep{Abdollahi2022,Ballet2023}) to search for the $\gamma$-ray emission from the magnetar Swift J1818.0-1607.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Data Set}
\label{sec:dataset} 

\begin{comment}
\begin{table}
    \setlength\tabcolsep{2.5pt}
    \centering
    \caption{Data set in Fermi analysis.}
    \label{tab:dataset}
    \scalebox{0.85}{
	\begin{tabular}{l|l} % four columns, alignment for each
		\hline
            Time span & Aug. 4, 2008 - Mar. 19, 2024 \\
            Energy band & 0.1 - 300 GeV \\
            Catalog & gll\_psc\_v34.fit (4FGL-DR4) \\
            IRFs & P8R3\_SOURCE\_V3 \\
            Components &\makecell[l]{0.1--0.3 GeV, zmax=90$^\circ$, evtype=16/32, enumbins=5;\\0.3--1 GeV, zmax=100$^\circ$, evtype=8/16/32, enumbins=6;\\1--300 GeV, zmax=105$^\circ$, evtype=4/8/16/32, enumbins=24.} \\
            ROI & 15$^\circ$ (20$^\circ$ source model) \\
            Free radius & 3$^\circ$ \\
            Galdiff & gll\_iem\_uw1216\_v13.fits \\
            Isodiff & iso\_P8R3\_SOURCE\_V3\_PSF0/1/2/3\_v1.txt \\
            Extended source template & 14 years \\
            Optimizer &\makecell[l]{MINUIT (default)\\ or NEWMINUIT (if failed when using MINUIT)}\\
            Fermitools & v2.2.0\\
            Fermipy & v1.2.0\\
		\hline
	\end{tabular}}
\end{table}
\end{comment}


We extracted approximately 15 years of Pass 8 data using the SOURCE event class within an energy range of 0.1--300 GeV and a 15$^\circ$ radius centered on the position of the Swift X-ray source Swift J1818.0-1607 [RA = 274.5010$^\circ$, Dec = -16.1314$^\circ$] \citep{Gronwall2020}. 
%
A standard event filter``\texttt{DATA\_QUAL>0 \&\& LAT\_CONFIG==1}'' has been employed to select data of good quality\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/data\_preparation.html}}. 
%
In order to retain the largest possible quantity of valid data while limiting the contamination from the Earth limb, the maximum zenith angle (Zmax) was set to 90$^\circ$, 100$^\circ$ and 105$^\circ$ for the low (0.1--0.3 GeV), medium (0.3--1 GeV), and high (1--300 GeV) energy intervals, respectively. 
%
Furthermore, the type of point spread functions (PSFs) for the three energy intervals mentioned were restricted to [PSF2 \& PSF3], [PSF1 \& PSF2 \& PSF3], and [PSF0 \& PSF1 \& PSF2 \& PSF3], respectively. 
%(evtype = 4, 8, 16, 32 represents PSF0, PSF1, PSF2, PSF3, respectively). 
%
Furthermore, the latest instrument response function (IRF), \texttt{P8R3\_SOURCE\_V3}, the 4FGL-DR4 catalog of \texttt{gll\_psc\_v34.fit}, and the 14-year extended source template were employed \citep{Ballet2023}, together with a 
%
rescaled \texttt{gll\_iem\_v07} interstellar emission model associated with the 4FGL-DR4 catalog (\texttt{gll\_iem\_uw1216\_v13.fits}). 
%
%We use the \texttt{Fermitools} package\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/software/}} (v.2.2.0) and \texttt{Fermipy} (v.1.2.0, \citet{Wood2017}),

%A summed likelihood analysis was performed in accordance with the mentioned settings. 
%employing the method of maximum likelihood estimation. 
%


We use the Test Statistic (TS) to measure the detection significance of gamma-ray radiation from a target source, 
$TS = 2(\log \mathcal{L}_{1} - \log \mathcal{L}_{0})$, where $\log \mathcal{L}_{1}$ and $\log \mathcal{L}_{0}$ are the logarithms of the maximum likelihood of the complete source model with and without the source (the "null hypothesis"), respectively \citep{Mattox1996}.
%
The square root of the TS value is approximately equal to the significance of detecting a given source. 


Given the proximity of this magnetar to the Galactic plane, and to prevent overestimation of the TS values for some sources (especially for sources with a soft spectrum), we have adopted a likelihood weighting approach as 
%
used in the creation of the 4FGL-DR3 and 4FGL-DR4 catalogs by the \lat collaboration \citep{Abdollahi2022}.
%
In light of the correlation between this weight and the photon energy and the type of PSF, we divided the photons into nine distinct components for the purpose of assigning the corresponding weight files and performing a summed likelihood analysis (later referred to as the weighted summed likelihood analysis), in a manner analogous to that employed by \citet{Abdollahi2022}\footnote{For details, please see 
\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/weighted\_like.pdf}}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Fit with 4FGL-DR4 Catalog}
\label{sec:DR4_only} 

% TS residual map (DR4 sources only)
\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{images/TSmap_residual_NotAdd_AddExcessAB.pdf}
    \caption{TS residual map of the ROI after considering only the sources contained in the 4FGL-DR4 catalog. Swift J1818.0-1607 is represented by a cyan circle situated at the center of the image, while two gamma-ray excesses, designated as Excess A and Excess B, are indicated by two yellow dashed ellipses. The $R_{95}$ of 4FGL J1816.2-1607 and the extension of 4FGL J1813.1-1737e are also plotted with a solid green ellipse and a circle, respectively. }
    \label{fig:tsmap_residual_dr4}
\end{figure}

A weighted summed likelihood analysis was performed using the \texttt{Fermitools} package\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/software/}} (v.2.2.0) and \texttt{Fermipy} package (v.1.2.0, \citet{Wood2017}), in accordance with the settings mentioned in Section \ref{sec:dataset}. 
%
Figure \ref{fig:tsmap_residual_dr4} presents the resulting TS residual map. 
%
Two distinct gamma-ray components are obvious. 
%
The fainter of the two, named Excess A, is situated in closer proximity to Swift J1818.0-1607, although it does not spatially coincide with it. 
%
In contrast, the brighter and more extended one, designated as Excess B, coincides with the \fermi extended source 4FGL J1813.1-1737e (which was, in fact, part of the model). 


In the 4FGL-DR4, 4FGL J1813.1-1737e is considered to be the potential GeV counterpart of HESS J1813-178, which was reported in the first HESS Galactic Plane Survey (HGPS) \citep{HESS2018} as a compact candidate PWN (Gaussian model with $\sigma=0.049\pm0.004^\circ$) powered by the pulsar PSR J1813-1749. 
%
The coordinates, spectral and spatial models adopted in the 4FGL-DR4 catalog for 4FGL J1813.1-1737e are [RA = 273.29$^\circ$, Dec = -17.62$^\circ$], LogParabola (LP), and a uniform disk model (RadialDisk) with a radius of $0.6^\circ$, respectively. 


Due to the considerable disparity in the spatial extensions of 4FGL J1813.1-1737e and HESS J1813-178, coupled with the incompatibility between their energy spectra, the potential correlation between them has been questioned by, e.g., \cite{HESS2024} and \cite{Guo2024}. 
%
In addition, \cite{HESS2024} reported on the detection of a new extended TeV source, HESS J1813-178B, which has an elongated Gaussian spatial model and a PL spectrum. 
%
These authors also updated the fits for the original compact HESS J1813-178 (called HESS J1813-178A)
after adding HESS J1813-178B. 


A \fermi point source, 4FGL J1816.2-1654c, is located between Excess A and Excess B as shown in Fig. \ref{fig:tsmap_residual_dr4}. 
%
4FGL J1816.2-1654c was first added to the \fermi catalog in 4FGL-DR2 \citep{Ballet2020} as a potential counterpart of PMN J1816-1649, a radio source detected in Parkes-MIT-NRAO (PMN) surveys \citep{Tasker1994}. 


The residual map shows that there is no significant excess at the position of the magnetar. 
%
However, the map of the residuals obtained with the quoted sources is complex and far from representing good fits for the region. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Unrepresented diffuse emission?}
\label{sec:MC} % used for referring to this section from elsewhere
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%
Here we shall explore whether an additional diffuse components help reduce the residuals. 
%
We do so because significant gas radiation is detected in the area where these $\gamma$-ray excesses exist, which has not been included in the present \fermi Galactic model.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{CO survey comparison}
\label{sec:CO} % used for referring to this section from elsewhere

\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{images/K_vs_V_12CO_MWISP.pdf}
    \caption{$^{12}$CO (J=1-0) spectra. The plot shows the average main beam brightness temperature ($T_{MB}$) of all pixels versus the radial velocity of the molecular gas in the region coincident with Excess A and B.}
    \label{fig:MC_spectra}
\end{figure}

\begin{figure*}
    \centering
        \includegraphics[width=0.66\columnwidth]{images/MC_12CO_0to29_AddExcessAB.pdf}
        \includegraphics[width=0.66\columnwidth]{images/MC_12CO_29to45_AddExcessAB.pdf}
        \includegraphics[width=0.66\columnwidth]{images/MC_12CO_45to65_AddExcessAB.pdf}
        \includegraphics[width=0.66\columnwidth]{images/COGAL_all_raw_0to29kms.pdf}
        \includegraphics[width=0.66\columnwidth]{images/COGAL_all_raw_29to45kms.pdf}
        \includegraphics[width=0.66\columnwidth]{images/COGAL_all_raw_45to65kms.pdf}
    \caption{Comparison of the $^{12}$CO ($J=0-1$) maps at different velocity ranges from the two different observations. The first row is from the MWISP project, which is used in this work. The botton row is from the composite surveys presented in \citep{Dame2001}, which are used in the \fermi Galactic model.}
    \label{fig:MC}
\end{figure*}

%\begin{figure}
%    \centering
%        \includegraphics[width=\columnwidth]{images/MC_12CO_45to65_Norm_BS_above50_AddContours_AddExcessAB.pdf}
%    \caption{CO map within the velocity range of 45-65 km/s from MWISP. This plot has been background suppressed and normalized.}
%    \label{fig:MC_45to65}
%\end{figure}

\subsubsection{MWISP}

We obtained data from the CO sky survey from the Milky Way Imaging Scroll Painting (MWISP) project \citep{MWISP}, (a $3^\circ \times 3^\circ$ square with the galactic center coordinate of $l=13.7^\circ$, $b=0^\circ$). 
% 
The $^{12}$CO image from MWISP spans a radial velocity of -150 to 250 km/s, with an angular resolution of $\sim 50''$ and a velocity resolution of 0.16 km/s\footnote{\url{https://cade.irap.omp.eu/dokuwiki/doku.php?id=mwisp}}. 
%
Molecular gas line radiation in a radial velocity range of 0 to 65 km/s is significant, as shown in Figure \ref{fig:MC_spectra}. 
%
There are three CO components with different velocity ranges ($0-29$ km/s, $29-45$ km/s, $45-65$ km/s), which can be fitted by a Gaussian having peak velocities of $19.33\pm2.29$, $38.44\pm3.95$, and $49.74\pm9.16$ km/s, respectively. 
%
In order to estimate the kinematic distances, we adopt the PowerLaw (PL) Milky Way rotation curve model
\begin{equation}
\theta(R) / \theta_{0}=1.022\left(R / R_{0}\right)^{0.0803}, 
\end{equation}
where $\theta(R)$ is the rotation velocity at the distance to the galactic center of $R$, $\theta_{0}$ and $R_{0}$ are the distance and rotation velocity of the Sun with $\theta_{0}$ = 240 km/s and $R_{0}$ = 8.34 kpc \citep{Russeil2017}. 
%
The resulting kinetic distances are $13.68-14.13$ or $2.17-2.62$ kpc, 
%for clouds with a peak velocity of $19.33\pm2.29$ km/s, 
$12.19-12.68$ or $3.62-4.11$ kpc, 
%for a peak velocity of $38.44\pm3.95$ km/s, 
and $11.40-12.30$ or $4.00-4.91$ kpc, for $0-29$ km/s, $29-45$ km/s, and $45-65$ km/s, respectively.
%for a peak velocity of $49.74\pm9.16$ km/s.


The $^{12}$CO maps in the three different velocity ranges for the selected region are shown in the top row of Figure \ref{fig:MC}. 
%
The enhancements found (from left to right) coincide with Excess A, the \fermi source 4FGL J1816.2-1654c, and Excess B, respectively. 


%The latest Galactic interstellar emission model used for the 4FGL catalog analysis (\fermi Galactic model) is provided on the \fermi official website\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/access/lat/BackgroundModels.html}}. 
%
%Since the results of the surveys of $^{12}$CO (J=1–0) are available, these observations have been widely used as a tracer of interstellar H$_2$ \citep{Fermi2016}. 
%


\subsubsection{\fermi Galactic model}

In the \fermi Galactic model\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/access/lat/BackgroundModels.html}}, a composite of 37 individual CO surveys \footnote{\url{https://lweb.cfa.harvard.edu/rtdc/CO/CompositeSurveys/}} presented in \cite{Dame2001} is adopted as one of the gas templates \citep{Fermi2016}. 
%
This composite has a resolution of approximately 9$^{\prime}$ FWHM at low latitudes and a velocity resolution of 1.3 km/s\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/software/aux/4fgl/Galactic_Diffuse_Emission_Model_for_the_4FGL_Catalog_Analysis.pdf}}. 
%
For comparison, we also extracted the $^{12}$CO data in the same three velocity ranges from the composite surveys and presented them in the bottom row of Figure \ref{fig:MC}. 
%
A comparison of the molecular cloud profiles in the two sets of CO maps reveals notable similarities, with the exception of those within the velocity range of 45-65 km/s, indicating that this component has not been incorporated into the current \fermi Galactic model. 
%
%Thus, a connection between the 45-65 km/s molecular clouds and the $\gamma$-ray excesses mentioned above is potentially possible. 
%
%We explored this possibility by adding a new source, which we shall name Cloud 45-65, assuming a SpatialMap model for it directly from the CO map within the velocity range of 45-65 km/s. 
%
%This map, which has been background suppressed and normalized according to the pipeline for extended source analysis\footnote{For details please see \url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/extended/extended.html}}, 
%is presented in Figure \ref{fig:MC_45to65} and will be used to build the SpatialMap model of Cloud 45-65.

%We explored this possibility by adding a new source, which we shall name Cloud 45-65, assuming a SpatialMap model for it directly from the CO map within the velocity range of 45-65 km/s. 
%
%This map, which has been background suppressed and normalized according to the pipeline for extended source analysis\footnote{For details please see \url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/extended/extended.html}}, 
%
We explored this possibility by introducing a new source, named Cloud 45-65, and modeling it using a SpatialMap model. 
%
The CO map within the velocity range of 45-65 km/s, following background suppression and normalization according to the extended source analysis pipeline\footnote{For details please see \url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/extended/extended.html}}, was used to construct the SpatialMap model for Cloud 45-65. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cloud 45-65}
\label{sec:Cloud45-65} % used for referring to this section from elsewhere

\begin{table*}
    \setlength\tabcolsep{4pt}
    \centering
    \caption{Results of the weighted summed likelihood analysis with Cloud 45-65 added.} 
    \label{tab:Cloud45-65}
    \scalebox{1.0}{
    \begin{tabular}{l|l:cc}
        \hline
        Source Model &Parameters & Cloud 45-65 &4FGL J1813.1-1737e \\\hline
        \multirow{9}*{\makecell[l]{4FGL J1813.1-1737e \\(2D Gaussian \& PL)\\\\Cloud 45-65\\(SpatialMap \& LP)}} 
            &Tolerance &$10^{-3}$ &- \\
            &$\Delta \mathcal{L}$ &335.84 &- \\
            &$\Delta$ AIC &-673.68 &- \\
            &TS &255.07 &202.10 \\
            &Flux ($10^{-8}$ ph cm$^{-2}$ s$^{-1}$) &$16.66\pm1.74$ &$14.56\pm2.25$ \\
            &Energy Flux ($10^{-11}$ erg cm$^{-2}$ s$^{-1}$) &$11.98\pm0.85$ &$13.01\pm0.99$ \\\cdashline{2-4}
            &Prefactor(P) / Norm(N) &N: $(2.44\pm0.25)\times10^{-10}$ &P: $(1.21\pm0.12)\times10^{-11}$ \\
            &Index(I) / $\alpha$ &$\alpha:1.53\pm0.07$ &I: $-2.13\pm0.04$ \\
            &Scale(S) / $\beta$  &$\beta:0.33\pm0.02$ &S: 1000 (fixed) \\
            &Eb &300 (fixed) &none \\\hline
    \end{tabular}}
\end{table*}

\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{images/TS_residual_4FGLJ1813_2DG_PL_MC4565_LP_AddContours_AddRegions.pdf}
    \caption{TS residual map when adding Cloud 45-65 and 4FGL J1813.1-1737e (assuming the SpatialMap and LP, and 2D Gaussian and PL, respectively).}
    \label{fig:TSmap_Cloud45-65}
\end{figure}

\begin{figure*}
    \centering
        \includegraphics[width=0.66\columnwidth]{images/FT_cloud_45-65_sed_4FGLJ1813_2DGaussian_PL_MC4565_SM_LP.png}   \includegraphics[width=0.66\columnwidth]{images/FT_4fgl_j1813.1-1737e_sed_4FGLJ1813_2DGaussian_PL_MC4565_SM_LP.png}
        \includegraphics[width=0.66\columnwidth]{images/4fgl_j1813.1-1737e_sed_NotAdd_MCC.png}
        \caption{SEDs of Cloud 45-65 (SpatialMap \& LP) and 4FGL J1813.1-1737e (2D Gaussian \& PL) resulting from the fitting after adding Cloud 45-65 and 4FGL J1813.1-1737e with updated spatial and spectral models to the source model. In the final panel, the SED of 4FGL J1813.1-1737e fitted directly with the 4FGL-DR4 catalog is presented for comparison.}
    \label{fig:SED_Cloud45-65}
\end{figure*}



As shown in the CO map of 45-65 km/s, Excess A, Excess B, 4FGL J1816.2-1654c and 4FGL J1813.1-1737e are located in the region where there is obvious gas emission. 
%
Since we try to explore the possibility of describing them simultaneously, 4FGL J1816.2-1654c and 4FGL J1813.1-1737e are removed from the source model file, and Cloud 45-65 with a spatial model of SpatialMap is added. 
%
In addition, the ROI is centered on the molecular cloud map ($l=13.7^\circ$, $b=0^\circ$). 
%
To assess improvements in fitting for the new ROI, a weighted summed likelihood analysis was conducted without adding or deleting any other sources from the source model file. 
%
We obtain a maximum log-likelihood ($\mathcal{L}$) of 636714.0 for the new ROI. 


We considered PL, LP, and ExpCutoff (EC) as possible spectra of Cloud 45-65.
%
The LP spectral model demonstrates superior performance and gives a TS of 1466.4 for Cloud 45-65 in our weighted summed likelihood analysis. 
%
However, the resulting TS residual map still shows a significant excess in the area of the original 4FGL J1813.1-1737e, and the fitted spectrum of Cloud 45-65 cannot describe its emission in the high-energy band (> 10 GeV). 
%
In addition, compared to the source model directly using the 4FGL-DR4 catalog, the Akaike information criterion (defined as $AIC=2(D.O.F.-\mathcal{L})$; \cite{Akaike1974}) is $\Delta AIC = -15.82$. 
%
Thus, 4FGL J1813.1-1737e is likely to be an independent extended source.

%Since a considerable portion of original 4FGL J18131.1-1737e is covered by Cloud 45-65, it is necessary to re-estimate its spatial model before undertaking a spectral fit. 
%An extension fit was conducted for 4FGL J1813.1-1737e with both the RadialDisk and RadialGaussian models. 
%The RadialGaussian model was determined to be superior, with a larger $TS_{ext}$ (greater than the previous by about 60).
%A 2D Gaussian model centered on [RA = $273.33 \pm 0.05^\circ$, Dec = $-17.57 \pm 0.05^\circ$], with $\sigma = 0.56 \pm 0.07^\circ$ was however reported as the best spatial model for 4FGL J1813.1-1737e by \cite{HESS2024} recently. 
%We tested both the 2D Gaussian and the fitted RadialGaussian spatial models for 4FGL J1813.1-1737e assuming the same PL spectral model. 
%The results obtained from this test also support the hypothesis that the 2D Gaussian is superior, as evidenced by a higher TS value for 4FGL J1813.1-1737e ($\Delta$ TS = 27.90) and $\Delta$ AIC = -25.90. 
%Thus, the 2D Gaussian was adopted as the optimum spatial model for 4FGL J1813.1-1737e, and we added it back to the source model file. 
%
We added 4FGL J1813.1-1737e back. 
%
%, assumed a PL spectrum, and tested three spatial models for it: RadialGaussian, RadialDisk, and the 2D Gaussian model reported in \cite{HESS2024}. As in \cite{HESS2024}, a 2D Gaussian model centered on [RA = $273.33 \pm 0.05^\circ$, Dec = $-17.57 \pm 0.05^\circ$], with $\sigma = 0.56 \pm 0.07^\circ$ is the best. 
%With these considerations, a weighted summed likelihood analysis was performed in the case of the PL or LP model for both 4FGL J1813.1-1737e and Cloud 45-65, respectively, and we obtained the best fit assuming a PL and LP model for 4FGL J1813.1-1737e and Cloud 45-65, respectively. 
We tested PL and LP spectra for both 4FGL J1813.1-1737e and Cloud 45-65, together with
a RadialGaussian, RadialDisk, and the 2D Gaussian model reported in \cite{HESS2024}. 
We obtained the best fit when assuming a PL for 4FGL J1813.1-1737e and a LP for Cloud 45-65. 
As in \cite{HESS2024}, we find that a 2D Gaussian model centered on [RA = $273.33 \pm 0.05^\circ$, Dec = $-17.57 \pm 0.05^\circ$], with $\sigma = 0.56 \pm 0.07^\circ$ is the best for 4FGL J1813.1-1737e. 
%
The detailed results of the corresponding weighted summed likelihood analysis are given in Table \ref{tab:Cloud45-65}. 
%
Figures \ref{fig:TSmap_Cloud45-65} and \ref{fig:SED_Cloud45-65} present the resulting TS residual map and the SEDs with 15 energy bins of Cloud 45-65 and 4FGL J1813.1-1737e. 
%
Compared to the fit with the source model directly from the 4FGL-DR4 catalog, the improvement in the fit is notable, with a much cleaner residual map and a prominent $\Delta AIC$ of -673.7. 
%
Both Excess B and the radiation attributed to the original 4FGL J1816.2-1654c can be fitted well with the newly incorporated diffuse emission of Cloud 45-65. 
%
The spectrum of Cloud 45-65 can be well described with a soft LP model as shown in the left panel of Figure \ref{fig:SED_Cloud45-65}, and its TS value is as high as 255.1 in the fit. 
%
The obtained SED of 4FGL J1813.1-1737e is fitted with a harder PL model and is also a better match to the spectra than the LP model in the 4FGL-DR4 catalog. 
%
Both are presented in the middle and right panels of Figure \ref{fig:SED_Cloud45-65}, respectively. 
%
%The harder spectrum of 4FGL J1813.1-1737e facilitates its connection to the spectrum of its potential TeV counterpart, HESS J1813-178B reported in \cite{HESS2024}. 


%Excess A is still visible, but this is expected because 
%there is obvious gas radiation at this position of Excess A only in the 29-45 km/s CO map, not in the 45-65 km/s map which is used to build the spatial model of 
%Cloud 45-65 does introduce any emission at its position.
%
%Given the observation that the gas radiation at the position of Excess A on the 29-45 km/s CO map from the MWISP is brighter than that on the corresponding map used to develop the \fermi Galactic model, it is hypothesized that Excess A originates from the background. 
%
Excess A remains visible, which is expected, as clear gas radiation at this location appears only in the 29–45 km/s CO map. Furthermore, the gas radiation exhibits greater intensity in MWISP, indicating that Excess A is likely attributable to background mismatch. 


%However, a considerably fainter and slightly extended Excess B, similar to Excess A, remains in the residual map, and it is spatially coincident with PSR J1813-1749 and its TeV PWN HESS J1813-178 (or HESS J1813-178B in \citet{HESS2024}). 
%
%Unlike Excess A, this component could potentially represent a new compact source rather than another contributor from the galactic background for the following two reasons. 
%
%First, there is no discernible gas radiation on the CO map of 29-45 km/s from both the MWISP and the composite surveys in {Dame2001} at the position of the weakened excess B. 
%
%Secondly, in this position, the detections of a point source in \citet{Araya2018}, a slightly extended Component A in \citet{Wach2023}, SrcB in \citet{Guo2024}, Component A and C in \citet{HESS2024} were reported. 
%
A fainter and slightly extended Excess B remains, coincident with PSR J1813–1749 and HESS J1813–178. Unlike Excess A, it may represent a new compact source, called Source B hereafter, given the lack of obvious gas emission at this position on the cloud map of 0-29 and 29-45 km/s. 


%However, it should be noted that although the additions of these sources are helpful in improving their fits for this region, except for SrcB in \citet{Guo2024}, all other detections are not significant enough to reach the detection threshold ($4\sigma$) for \fermi sources even in their unweighted likelihood analyses. 
%
%This method is found to possibly result in an overestimation of the TS value for a source, especially for extended and soft sources in close proximity to the Galactic plane. 
%
%This potential new source is henceforth designated as Source B, and it may be the GeV counterpart of HESS J1813-178 (or HESS J1813-178B). 
%
%In the following section, we perform a more thorough analysis to test this hypothesis. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Is Excess B a new source?}
\label{sec:SourceB} % used for referring to this section from elsewhere

\begin{table} 
    \setlength\tabcolsep{2pt}
    \centering
    \caption{Localization and extension tests for Source B (all assuming a PL spectrum).}
    \label{tab:localize_SourceB}
    \scalebox{1.0}{
        \begin{tabular}{l|cccccc}
            \hline
            Spatial Model &RA ($^\circ$) &Dec ($^\circ$) &$R_{95}$ ($^\circ$) &$R_{68}$ ($^\circ$) &$R_{68err}$ ($^\circ$) &$TS_{ext}$ \\\hline
            PointSource &273.4671 &-17.8523 &0.0871 &none &none &none \\
            RadialDisk &273.5060 &-17.8291 &none &0.1469 &0.0238 &12.7355 \\
            RadialGaussian &273.4950 &-17.8375 &none &0.1390 &0.0268 &13.1775\\
            \hline
        \end{tabular}}
\end{table}

\begin{table*}
    \setlength\tabcolsep{4pt}
    \centering
    \caption{Results of the weighted summed likelihood analysis with Cloud 45-65 and Source B added. } 
    \label{tab:SourceB}
    \scalebox{1.0}{
    \begin{tabular}{l|l:ccc}
        \hline
        Source Model &Parameters & Cloud 45-65 &4FGL J1813.1-1737e &Source B \\\hline
        \multirow{9}*{\makecell[l]{4FGL J1813.1-1737e\\(2D Gaussian \& PL)\\\\Cloud 45-65\\(SpatialMap \& LP)\\\\Source B\\(PointSource \& LP)}} 
            &Tolerance &$10^{-3}$ &- &-  \\%\cdashline{2-5}
            &$\Delta \mathcal{L}$ &384.38 &- &- \\%\cdashline{2-5}
            &$\Delta$ AIC &-762.76 &- &- \\%\cdashline{2-5}
            &TS &185.98 &199.16 &38.27 \\%\cdashline{2-5}
            &Flux ($10^{-8}$ ph cm$^{-2}$ s$^{-1}$) &$13.71\pm1.51$ &$17.29\pm2.53$ &$0.46\pm0.34$ \\%\cdashline{2-5}
            &Energy Flux ($10^{-11}$ erg cm$^{-2}$ s$^{-1}$) &$10.54\pm0.82$ &$13.43\pm1.03$ &$1.19\pm0.25$ \\\cdashline{2-5}
            &Prefactor(P) / Norm(N) &N: $(2.08\pm0.24)\times10^{-10}$ &P: $(1.32\pm0.12)\times10^{-11}$ &P: $(5.88\pm3.30)\times10^{-13}$ \\
            &Index(I) / $\alpha$ &$\alpha:1.35\pm0.07$ &I: $-2.19\pm0.04$ &I: $-1.80\pm0.17$ \\
            &Scale(S) / $\beta$  &$\beta:0.40\pm0.03$ &S: 1000 (fixed) &S: 1000 (fixed) \\
            &Eb &300 (fixed) &none &none \\\hline
    \end{tabular}}
\end{table*}

\begin{figure*}
    \centering
        \includegraphics[width=.66\columnwidth]{images/FT_cloud_45-65_sed_SrcB_PS_PL_4FGLJ1813_2DGaussian_PL_MC4565_SM_LP.png}   \includegraphics[width=.66\columnwidth]{images/FT_4fgl_j1813.1-1737e_sed_SrcB_PS_PL_4FGLJ1813_2DGaussian_PL_MC4565_SM_LP.png}
        \includegraphics[width=.66\columnwidth]{images/FT_source_b_sed_SrcB_PS_PL_4FGLJ1813_2DGaussian_PL_MC4565_SM_LP_8bins.png}  
        \includegraphics[width=\columnwidth]{images/SED_SrcB_PS_PL_4FGLJ1813_2DG_PL_MC4565_LP_4FGLJ1813andHESSB_8bins.pdf}
        \includegraphics[width=\columnwidth]{images/SED_SrcB_PS_PL_4FGLJ1813_2DG_PL_MC4565_LP_SrcBandHESSA_8bins.pdf} 
        \caption{Top: SEDs of Cloud 45-65 (SpatialMap \& LP), 4FGL J1813.1-1737e (2D Gaussian \& PL) and Source B (PointSource \& PL) resulting from the fitting after adding Cloud 45-65, 4FGL J1813.1-1737e with updated spatial and spectral models, and Source B to the source model file. 
        Bottom: The SEDs of 4FGL J1813.1-1737e (in this work) and its potential TeV counterpart, HESS J1813-178B (derived from \citet{HESS2024}), are plotted together and presented in the left panel for comparison. The right panel is the same plot for Source B (in this work) and HESS J1813-178A (from \citet{HESS2024}). The \textit{JA} in the figure represents the joint analysis with \lat and \hess data in \citet{HESS2024}, in which $\sigma_M$ [$\sigma$] of HESS J1813-178B [HESS J1813-178A] is $0.54 \pm 0.003^\circ$ [$0.056 \pm 0.003^\circ$]. The \textit{HA} represents the analysis with \hess data alone in \citet{HESS2024}, in which $\sigma_M$ [$\sigma$] of HESS J1813-178B [HESS J1813-178A] is $0.72 \pm 0.08^\circ$ [$0.056 \pm 0.003^\circ$]. }
    \label{fig:SED_SourceB}
\end{figure*}

\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{images/TS_residual_SrcB_PS_PL_4FGLJ1813_2DG_PL_MC4565_LP_AddContours_AddRegions_AddTeV.pdf}
    \caption{TS residual map and TS excess map of 4FGL J1813.1-1737e (RadialDisk \& LogParabola) resulting from the weighted summed likelihood analysis when adding two new Fermi sources. PSR J1813-1749, HESS J1813-178A, HESS J1813-178B, and 2HWC J1814-173 are also noted but not involved in fitting.}
    \label{fig:TSmap_SourceB}
\end{figure}


The location and size of Excess B suggest that it could be a counterpart of HESS J1813–178 (HESS J1813–178A). 
To explore this possibility, we incorporated a new Source B into the model. 
%
Assuming a PL spectrum, the results of the localization and extension fits with the \texttt{localize} and \texttt{extension} tools integrated in \texttt{Fermipy} are presented in Table \ref{tab:localize_SourceB}. 
%
The highest TS$_{ext}$ is only $\sim 14$
%13.1775 undser 
%the assumption of a RadialGaussian model, 
so there is insufficient evidence to support an extended source model for Source B. 
%
%The coordinate of Source B with a PointSource model is [RA = $273.4671^\circ$, Dec = $-17.8523^\circ$] with an R$_{95}$ of $0.0871^\circ$ in our localization fit. 
The coordinates of Source B assuming a PointSource model are [RA = $273.5^\circ$, Dec = $-17.9^\circ$], with an uncertainty R$_{95}$ of $0.09^\circ$. 
%[RA = $273.4671^\circ$, Dec = $-17.8523^\circ$], with an uncertainty R$_{95}$ of $0.0871^\circ$. 
%
%This spatial model is adopted in the following spectral analyses. < is obvious




% up to here Diego.
We tested both the PL and the LP spectral models for Source B, but there is barely any difference in the $\Delta \mathcal{L}$ and TS values. 
%
The results of the weighted summed likelihood analysis are presented in Table \ref{tab:SourceB}.
%

With Source B incorporated, there is a notable enhancement in the fit for this region, with a $\Delta \mathcal{L}$ of 384.38 and a $\Delta$ AIC of -762.76 compared to the fitting results before adding Cloud 45-65 and Source B. 
%
Even compared to the results obtained with the addition of Cloud 45-65 alone, the values of $\Delta \mathcal{L}$ and $\Delta$ AIC are increased / reduced by about 50 and 90, respectively. 
%
Cloud 45-65, 4FGL J1813.1-1737e, and Source B are significant, with a TS value of 186.0, 199.1 and 38.3, respectively. 
%
The resulting TS residual map and SEDs of Cloud 45-65, Source B, and 4FGL J1813.1-1737e with updated spatial and spectral models are presented in Figures \ref{fig:TSmap_SourceB} and \ref{fig:SED_SourceB}, respectively. 
%
%The resulting TS residual map and SEDs of Cloud 45-65, Source B, and 4FGL J1813.1-1737e with updated spatial and spectral models are presented in Figures \ref{fig:TSmap_SourceB} and \ref{fig:SED_SourceB}, respectively. 
%
%As demonstrated in these maps, the incorporation of two additional sources, Cloud 45-65 and Source B, has resulted in a significant improvement in the fit to the GeV radiation observed, including Excess B and the emission that was previously attributed to 4FGL J1816.2-1654c. 
%
Unsurprisingly, Excess A cannot still be fitted well.


These results suggest that Cloud 45-65 is associated with molecular clouds with a velocity range of $45-65$ km/s. 
%
Its GeV emission is predominantly concentrated within an energy range of less than 10 GeV, which can be effectively described by an LP model. 
%
Another point like source, Source B, exhibits spatial coincidence with PSR J1813-1749, HESS J1813-178A, and the composite SNR G12.8-0.0. 
%
As demonstrated in Figure \ref{fig:SED_SourceB}, the GeV radiation of Source B can be modeled with a simple PL model, which connects to the spectrum of a TeV PWN, HESS J1813-178A. Furthermore, the combined spectrum of these two sources is consistent with the observed gamma-ray spectrum in young PWNe. 
%
In the case of 4FGL J1813.1-1737e, with an updated 2D Gaussian model, a harder PL spectral model shows superiority, also matching the spectrum of its potential TeV counterpart, HESS J1813-178B. 




%In conclusion, the addition of Cloud 45-65 and Source B, and the update on the spatial and spectral models of 4FGL J1813.1-1737e improve the fitting for the $\gamma$-ray radiation in this region, and all of them are significant. Cloud 45-65 should be associated with molecular clouds with a velocity range of 45-65 km/s. Regarding the other two sources, our results indicate that, in addition to spatial coincidence, their spectra also support the correlation between Source B and HESS J1813-178A, as well as between 4FGL J1813.1-1737e and HESS J1813-178B. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sources not absorbed by a diffuse normalization mismatch}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We have finally investigated the impact of the uncertainty in the normalization of the galactic diffuse model. This was achieved by fixing the normalization of the galactic diffuse to 0.94 and 1.06 times (i.e., $\pm$6\%) of the fitted values before adding two new extended sources, Cloud 45-65 and Source B, in the input source model. 
%
Subsequently, a weighted summed likelihood analysis was performed. 
%
The TS values of these two sources remain notably high, with a minimum of 173.44 for Cloud 45-65 and 32.32 for Source B, indicating that they  
%
cannot be attributed to the uncertainty in the galactic diffuse normalization.








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Concluding remarks}
\label{sec:Conclusion} % used for referring to this section from elsewhere
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%After comparing several spectral and spatial models, which are common for \fermi sources, for Cloud 45-65 and Source B, we found that LP \& SpatialMap and PL \& PointSource are the optimum model conjunction for them, respectively. 
%In addition, PL \& 2D Gaussian are superior to the LP \& RadialGaussian, which are adopted in 4FGL-DR4, for 4FGL J1813.1-1737e. 
%The $\gamma$-ray emission, which was attributed to 4FGL J1816.2-1654c, fits well with Cloud 45-65. 
%This suggests that 4FGL J1816.2-1654 probably originates from the galactic background instead of an independent source. 
%
%With these considerations, we obtained a much better source model for this region with $\Delta AIC=-762.76$. 
%
%In this work, we derived the best and most plausible source model for the MeV-GeV emission from the region near Swift J1818.0-1607 with $\Delta AIC=-762.76$. 
%We obtained significant detections of two new \fermi sources, Cloud 45-65 and Source B, with TS values of 185.98 and 38.27, respectively. 
%In addition, we found PL \& 2D Gaussian is more suitable for 4FGL J1813.1-1737e. 
%
%
%Cloud 45-65 should come from the interaction between the CR and the molecular clouds of 45-65 km/s. 
%In light of spatial and spectral matching, Source B and 4FGL J1813.1-1737e may be the GeV counterpart of HESS J1813-178B and HESS J1813-178B, respectively. 
%4FGL J1820.4-1609c is likely come from the galactic background too. 
%The associations between the sources detected in this region by different devices are discussed. 
%
%Finally, this work demonstrates the significant impact of the radiation from molecular clouds / background on the correct understanding and analysis of the sky. 
%It also exemplifies the impact of incorporating weights on the TS value estimate, particularly for extended sources or sources with a soft spectrum, such as 4FGL J1813.1-1737e and Cloud 45-65, whose TS values are overestimated by several hundred in the unweighted case.
%
%
In this study, we derived the most plausible source model for the MeV-GeV emission from the region near Swift J1818.0-1607, with a $\Delta AIC = -762.76$. 
%
Our analyses led to the detection of two new \fermi sources, Cloud 45-65 and Source B, with TS values of 185.98 and 38.27, respectively. 
%
We associated 4FGL J1820.4-1609c with the galactic background and found that a PL \& 2D Gaussian model better describes 4FGL J1813.1-1737e. 

Cloud 45-65 likely results from CR interactions with molecular clouds of 45-65 km/s. 
%
Based on spatial and spectral matching, we propose Source B and 4FGL J1813.1-1737e as the GeV counterparts of HESS J1813-178A and HESS J1813-178B, respectively. 
%
We also discussed the associations between more sources detected by different instruments in this region. 


Furthermore, our work highlights the significant impact of molecular clouds / background radiation on \fermi analyses. 
%
It also emphasizes the importance of incorporating weights in TS value estimation, particularly for extended and soft-spectrum sources like 4FGL J1813.1-1737e and Cloud 45-65, which are overestimated by several hundred in the unweighted case. 


